Towards Fast, Accurate and Stable 3D Dense Face Alignment

Existing methods of 3D dense face alignment mainly concentrate on accuracy, thus limiting the scope of their practical applications. In this paper, we propose a novel regression framework named 3DDFA-V2 which makes a balance among speed, accuracy and stability. Firstly, on the basis of a lightweight backbone, we propose a meta-joint optimization strategy to dynamically regress a small set of 3DMM parameters, which greatly enhances speed and accuracy simultaneously. To further improve the stability on videos, we present a virtual synthesis method to transform one still image to a short-video which incorporates in-plane and out-of-plane face moving. On the premise of high accuracy and stability, 3DDFA-V2 runs at over 50fps on a single CPU core and outperforms other state-of-the-art heavy models simultaneously. Experiments on several challenging datasets validate the efficiency of our method. Pre-trained models and code are available at https://github.com/cleardusk/3DDFA_V2.

==> related.tex <==
% [todo: refine it and compare it with the methods proposed by this paper]
%\vspace{-0.4cm}
\section{Related work}
We review related works from three aspects: Face Alignment, 3D Face Reconstruction and Video-based Face Alignment.
\subsection{Face Alignment}
Face alignment can be modelled as a regression problem where a set of 2D facial fiducial landmarks are located automatically.
Traditional methods are mainly based on model fitting, including Active Appearance Model(AMM)~\cite{cootes2001active}, Active Shape Model (ASM)~\cite{cootes1995active} and Constrained Local Model (CLM)~\cite{cristinacce2006feature}.
AAM methods~\cite{matthews2004active,saragih2007nonlinear,tzimiropoulos2013optimization} perform alignment through minimizing the appearance difference between the input image and the shape model. ASM~\cite{cootes1995active} and CLM methods~\cite{kim2013deformable,asthana2013robust} build a template model for each landmark and use a PCA shape model to constrain the fitting results. Then cascaded regression~\cite{dollar2010cascaded,xiong2015global} and CNN-based methods~\cite{bulat2017far,liang2015unconstrained,peng2016recurrent} are preferred and achieve the-state-of-the-art performance.
\textbf{Large Pose Face Alignment.}
For large-pose faces, 3DMM has been shown as an effective and strong prior~\cite{zhu2016face,jourabloo2015pose}. Therefore, fitting a 3D face model to a single 2D image gains attention for large pose face alignment~\cite{jourabloo2016large,zhu2016face,liu2016joint,mcdonagh2016joint,jourabloo2017pose}. Among these prior works, iterative approaches with a cascade of regressors are preferred. At each cascade, there is a single~\cite{tulyakov2015regressing} or two regressors~\cite{wu2015robust} used to improve the performance.
Recently, the works in~\cite{bulat2016two,bulat2017far} choose to directly regress the heatmap to perform face alignment and achieve state-of-the-art performance.

\if 0
\textbf{Dense Face Alignment.} As the sparse face alignment has been highly completed by previous methods, the dense face alignment develops. It is to note that dense alignment should provide the dense correspondence from the input face image to 3D facial reference geometry. Liu et al. ~\cite{liu2017dense} adopt multiple constraints to train a CNN to estimate the 3D face shape, which provides a very dense 3D alignment. The works in~\cite{alp2017densereg,yu2017learning} directly learn a mapping from the input image into a 3D template grid through a fully convolutional network,  but those predicted correspondence is not complete and only visible face-region is considered.
\fi

% todo: the relationship between 3d face reconstruction and 3d dense face alignment
\subsection{3D Face Reconstruction}
%The 3D face reconstruction from a single image in-the-wild draws a lot of interest because of its wide applications.
\textbf{Model-based Methods.} The 3DMM firstly proposed by Blanz et al.~\cite{blanz1999morphable} is the foundation of model-based methods for 3D face reconstruction. Most of earlier methods first establish the correspondences between input faces and landmarks~\cite{zhu2015high,huber2016multiresolution,lee2012single,thies2016face2face,cao2014displaced,grewe2016fully} or feature points~\cite{grewe2016fully,romdhani2005estimating}, then try to solve the non-linear optimization to estimate the 3DMM coefficients. However, these methods are very sensitive to the accuracy of landmarks or other feature points.
%In the meanwhile, several methods~\cite{alp2017densereg,yu2017learning} adopt CNN to regress the dense correspondence between the input image and 3D template, then estimate the 3DMM parameters under the regressed dense constraints.
Recently, several works exploit CNN to directly regress the 3DMM parameters, including cascaded CNN structure~\cite{jourabloo2016large,zhu2016face,richardson20163d,liu2016joint} and end-to-end structure~\cite{dou2017end,tuan2017regressing}. In addition, unsupervised methods~\cite{tewari2017mofa,bas20173d} have been exploited recently, but the performance degrades rapidly under large-poses and unbalanced illuminations.

% VRN, PRNet
\textbf{Regression-based Methods.} VRN~\cite{jackson2017large} performs the direct regression of a volumetric representation of the 3D facial geometry from a single face. PRNet~\cite{feng2018joint} designs a 2D representation named UV position map to record the 3D shape of a face, then adopts an end-to-end CNN structure to directly regress it. Although these methods achieve state-of-the-art performance, they greatly rely on the fully convolutional network to ensure the resolution of predicted volumetric or UV map, which makes these methods slow and memory-consuming.
%
\if 0
\subsection{Video-based Face Alignment} Video-based face alignment estimates facial landmarks in video sequences~\cite{liu2010video}. Apart from the accuracy of landmarks, stabilization is also an important evaluation metric for video-based alignment. Peng et al.~\cite{peng2016recurrent} propose to incorporate a sequence of spatial and temporal recurrences for sequential face alignment in videos. Liu et al.~\cite{liu2018two} propose a Two-Stream Transformer Networks (TSTN) approach, which captures the complementary information of both the spatial appearance on still frames and the temporal consistency information across frames.
In ~\cite{dong2018supervision}, an unsupervised approach is proposed to use optical flow as a source of supervision, based on the observation landmarks in adjacent frames should be coherent with the optical flow.
 The recent work~\cite{tai2018towards} adopts a Fractional Heatmap Regression (FHR) for high-resolution video-based face alignment and proposes two constraints to address time delay and non-smooth issues for stability. % todo: write the drawback or the difference between our methods and theirs.
 \fi

